GerPS-Compare: Comparing NER methods for legal norm analysis

We apply NER to a particular sub-genre of legal texts in German: the genre of legal norms regulating administrative processes in public service administration. The analysis of such texts involves identifying stretches of text that instantiate one of ten classes identified by public service administration professionals. We investigate and compare three methods for performing Named Entity Recognition (NER) to detect these classes: a Rule-based system, deep discriminative models, and a deep generative model. Our results show that Deep Discriminative models outperform both the Rule-based system as well as the Deep Generative model, the latter two roughly performing equally well, outperforming each other in different classes. The main cause for this somewhat surprising result is arguably the fact that the classes used in the analysis are semantically and syntactically heterogeneous, in contrast to the classes used in more standard NER tasks. Deep Discriminative models appear to be better equipped for dealing with this heterogenerity than both generic LLMs and human linguists designing rule-based NER systems.

==> content/discussion.tex <==
% I deleted this page because discussion was also present in the results

==> content/introduction_old.tex <==
Public administration institutions follow processes based on legislation (e.g., laws and ordinances), when delivering a public service like car registration to citizens or companies. In Germany, the Federal Information Management (FIM)\footnote{\url{https://fimportal.de/glossar}} provides standardized methods for analyzing such legal bases. Trained public administration employees mark relevant terms or sentences of classes, such as the main actor as well as the result receiver, and create a list of discovered process steps together with the related data fields\footnote{Data fields represent the different pieces of information of online forms (e.g., first name, profession) that are necessary for the result receiver to apply for a service.}. Finally, they assemble all these elements in a process using a restricted and an extended BPMN\footnote{\url{https://www.bpmn.de/lexikon/bpmn/}} notation. This process is used to create web forms allowing an online delivery of the service for potential applicants. 
In this way, the service, the associated process, and data fields matching specific process steps are described on the basis of the associated legal basis. This annotation of legal texts with classes is called the FIM --- legal norm analysis, which represents the first step in the creation of administrative services with the identification of all involved process elements (e.g., steps or actors).\\
% The project ``Computer-assisted analysis of electronically available legal norms (Canarėno)'' of the ``Open Design of Digital Administrative Architectures (openDVA)''\footnote{\url{www.opendva.de}} working group is one of three research projects investigating the path from the legal text to its digital implementation and how it can be simplified and partially automated, both for new or existing legal texts and for their amendment while complying with and extending existing standards, as outlined in our vision by Mauch et al.~\cite{mauch2024IRIS}.

%We investigate and compare three methods for performing Named Entity Recognition (NER) to detect the classes relevant to the norm analysis, namely a rule-based (symbolic AI), a deep discriminative and a deep generative approach.
We investigate and compare three methods for performing Named Entity Recognition (NER) to detect the classes relevant to the norm analysis:
% I moved this from concept
\textbf{Rule-based methods}~\citep{10.1145/3445965}: Are approaches that resort to predefined patterns to detect class mentions in the text. They typically rely on regular expressions to build rules or external ressources to retrieve potential class candidates e.g., knowledge bases or glossaries. They are, in general, useful for classes with well defined structures, which makes them too inflexible for detecting complex and changing classes. This is why we also investigate the following two types of machine learning-based methods.
\textbf{Deep discriminative models}~\citep{premasiri-etal-2023-deep}: are machine learning models that aim at assigning classes to the input data by modeling the decision boundary between those classes. Discriminative models are generally used for e.g., NER or question answering e.g., BERT~\cite{devlin2019bert}.
They are usually used in the context of supervised learning and thus need a significant amount of annotated training data.
\textbf{Deep generative models}~\citep{8354080}: Are machine learning models that can generate new data instances that are similar to some seen training data. They are mainly trained using only a small number of examples (few-shot learning \todo{add reference?}). They try to understand the data distribution, in constract to discriminative models that are designed to perform classification tasks.
Generative models are used e.g., for image or text generation e.g., OpenAI GPT-4~\cite{openai2023gpt4}.


% text before rewrite ( - robin)
%Our goal is to select for each class the best-performing alternative and combine the approaches in a currently developed tool for supporting human annotators. In the following, we give more details about our experiments and results using the previously defined three methods to solve the NER task in the context of the legal norm analysis.

Our goal is to compare the different approaches and determine for each class which approach is performing the best. We do this in the light of a tool that we are developing in our working group. The use case of this tool - supporting human annotators - also guides part of our evaluation method. This comparison will be influence which approach will be implemented as part of this tool, or if multiple approaches should be combined.
In the following, we provide more details about our experiments and results using the previously defined methods to solve the NER task in the context of the legal norm analysis.

% maybe also rewrite the last sentence / closing sentence to better reflect the structure of the paper


==> content/related_work_discriminative.tex <==
\todo{abbreviations and language}
\todo{sort by time or content/architecture?}
\todo{check if BERT citation already included before}
\todo{remove repetitive citations for German LER dataset?}

\cite{Leitner_2020} present a relatively large newly created 
dataset for German legal NER (German LER dataset) and also evaluate the performance 
of multiple differently configured BiLSTM-CRF models on this dataset.

% note: arxiv
\cite{darjiGermanBERTModel2023} fine-tuned a German BERT model on
the German LER dataset \cite{Leitner_2020} and 
present their results that are better than the results originally achieved 
by \cite{Leitner_2020} when presenting the dataset.


\cite{Zollner_2021} used, among others, the German LER 
dataset \cite{Leitner_2020} when they compared the 
effect of different pre-training techniques for small BERT models and presented 
modified fine-tuning processes which resulted in performance improvements.



\cite{erd2022evaluation} used the same two architectures that will also 
be used in this paper (BiLSTM-CRF, XLM-RoBERTa \cite{Conneau_2019}) to evaluate and compare the 
performance improvements that different data augmentation methods and their 
combinations might achieve for NER tasks in the German legal domain.


% looks like this is just some internal publication
% they only use 2 classes (law references and references to court decisions)
\todo{warning: uni publisher}
\cite{peikert2022extracting} compare the performance of different approaches for 
the task of NER in the German legal domain. Among others, they evaluate BERT, 
BiLSTM-CRF, plain CRF and pattern-matching approaches. They created their own datasets for 
benchmarking, but used the German LER dataset \cite{Leitner_2020} for training.


% this is a more complex scenario, and more removed from what we do
% didnt quite understand what they do yet, will look into it more closely if determined relevant
\cite{smuadu2022legal} present a new architecture for multi-task domain adaption that 
involves a BERT layer, BiLSTM networks and Conditional Random Fields. They evaluate their 
approach on both Romanian and German legal datasets. 
% https://aclanthology.org/2022.nllp-1.29.pdf 

==> content/related_work_generative.tex <==
We describe related work for deep generative models for NER on legal texts in~\cite{Bachinger2024}. In addition, for LegalLens,~\cite{bernsohn-etal-2024-legallens} compared BERT models with open source LLMs on the domain of legal violation identification. 
\cite{joshi-etal-2024-il} proposed ``IL-TUR, a benchmark for Indian Legal Text Understanding and Reasoning'' and proposed among other things a LLM-based pipeline for the benchmark. 
With LAiW, \cite{dai2023laiw} propose a benchmark for Chinese legal LLMs. 


==> content/related_work_rulebased.tex <==
The application of Natural Language Processing (NLP) to legal texts is a relatively new development,
starting in an era where deep discriminative approaches to NER
have already been established as state of the art technologies.
Hence, many implementations of NER for legal documents in German
turn to deep discriminative ML approaches directly,
without systematically comparing these technologies to rule-based systems, 
as can bee seen in the references reviewed in the previous sections. 
Rule-based approaches to NER in legal documents
are mostly developed for languages lacking robust resources for ML development,
such as Afan Oromo \cite{m.e.phd.professordepartmentofcomputerscienceambouniversityamboethiopiaNLPRuleBased2019}
or Arabic \cite{abdallahIntegratingRuleBasedSystem2012}. 
The latter work stands out
by combining a rule-based approach with machine learning
and evaluating the effectiveness of both approaches.
The authors find
that the combined approach improves the F1-score
by $8-14\%$ compared to either the rule-based appraoch
or the machine learning approach alone.

A recent systematic comparison of a rule-based NER system
with deep learning and transfer learning systems can be found in
\cite{gorinskiNamedEntityRecognition2019},
dealing with the domain of electronic health records
rather than legal documents. 
They found that the hand crafted rule-based system
consistently outperforms both
the transfer learning and the deep leraning systems,
reaching an overall F1-score of $0.95$.
These results are in stark contrast with our results,
where the rule-based system for the German FIM-class recognition
reaches an overall micro F1-score of $0.56$ (macro F1: $0.50$). 
However,
these differences in F1-score results
must be seen in the context of differences in the design
and implementation of the respective rule-based systems:

\begin{enumerate}
\item The rule-based system described by \cite{gorinskiNamedEntityRecognition2019}
  comprises of a fully hand-crafted pipeline
  from raw input text to shallow syntactic analysis,
  made by domain experts.
  Our system implements only parts of this pipeline,
  relying on Spacy models for tokenization and morphology,
  and excluding syntactic analysis.
  These implementation decisions where motivated at least in part 
  by the project's desire to re-use existing technologies as much as possible
  in order to come up with an easy to implement system for practical application
  in public administration. 
\item Gorinski et al's rule-based system is based on entity definitions
  based on homogenous semantic types as developed by linguistic domain experts.
  The entity definitions used in our system
  are not solely based on natural semantic types,
  but are driven by the classes used in the FIM-based legal norm analysis.
  These classes are not always semantically homogenous.
  For instance,
  the class \emph{Signalwort} is defined as marking linguistic expressions
  indicating the degree of obligatoriness of a decision
  made on the basis of this statute.
  Most typically, this is indicated by modal verbs
  or the \emph{zu--}infinitive in its modal use.
  However,
  adjectives and adverbs such as \emph{angemessen} `appropriate'
  or \emph{berechtigt} `being eligible'
  and phrases such as \emph{auf Wunsch} `if desired'
  can also mark the degree of obligatoriness. 
\end{enumerate}


